Rank Reversal in Multilingual LLM Judges: A Label-Free Double-Centering Calibrator

Multilingual LLM judges produce different evaluator-backbone rankings depending on the prompt language: on an eight-language Agent-as-a-Judge benchmark, the top-ranked backbone alternates across English, Arabic, Chinese, Hindi, Japanese, Spanish, Turkish, and Swahili, and 7 of 15 backbone pairs show statistically significant pairwise rank reversal. We treat this as a measurement problem. The multilingual judge score decomposes additively into task difficulty, backbone skill, and a language-backbone interaction term, the last of which is recoverable without human labels by double-centering the cell-mean score matrix. We make this estimator (\textbf{Consensus-Based Calibration}, CBC) explicit, give an $O(1/\sqrt{n})$ finite-sample concentration bound with variance constant $(1-\tfrac{1}{m})(1-\tfrac{1}{k})$, and show that it is unbiased even when task-language interactions are present. Across 7{,}920 judge runs (6 backbones, 8 languages, 55 tasks, 3 frameworks), CBC raises held-out cross-task rank consistency $\tau$ from 0.650 to 0.902 and agrees with the held-out additive-model oracle in 100\% of per-language decisions versus 68.5\% raw; these are consistency diagnostics, not human-grounded correctness measures. On a separately collected M-RewardBench panel (7 languages, 1{,}500 items per language, 10{,}500 language-item instances, 5 evaluators), panel agreement with the public human gold preferences rises from 68.7\% to 76.6\% (gain 7.9 percentage points, 95\% CI $[6.0, 9.9]$), our strongest external evidence of downstream usefulness. The estimator is the standard two-way ANOVA interaction-recovery operation under sum-to-zero contrasts; our contribution is its application as a label-free post-hoc calibrator for multilingual LLM judges, an explicit finite-sample concentration bound, and an unbiasedness result that holds even under task-language misspecification.

==> Makefile <==
#===============================================================================
# Kurban Intelligence Lab -- paper build
#
#   make          build main.pdf (pdflatex -> bibtex -> pdflatex x2)
#   make arxiv    arxiv-submission.tar.gz, ready to upload
#   make blind    main-blind.pdf   (double-blind: no authors, no logo, no acks)
#   make logo     regenerate every logo asset from the vector master
#   make figures  regenerate the example figure
#   make clean    remove build artefacts (keeps the PDFs)
#   make purge    remove everything generated
#===============================================================================
MAIN  := main
LATEX := pdflatex -interaction=nonstopmode -halt-on-error

.PHONY: all arxiv blind logo figures clean purge
all: $(MAIN).pdf

$(MAIN).pdf: $(MAIN).tex kurbanlab.sty affiliations.tex references.bib
	$(LATEX) $(MAIN)
	-bibtex $(MAIN)
	$(LATEX) $(MAIN)
	$(LATEX) $(MAIN)
	@echo "==> $(MAIN).pdf"

# arXiv wants the .bbl, not the .bib, and no build cruft.
arxiv: $(MAIN).pdf
	@rm -rf arxiv && mkdir -p arxiv/figures arxiv/logo
	@cp $(MAIN).tex kurbanlab.sty affiliations.tex references.bib .latexmkrc $(MAIN).bbl arxiv/
	@cp figures/*.pdf arxiv/figures/ 2>/dev/null || true
	@mkdir -p arxiv/analysis
	@cp analysis/*.png arxiv/analysis/ 2>/dev/null || true
	@cp logo/kil-lockup.pdf arxiv/logo/ 2>/dev/null || true
	@cd arxiv && tar czf ../arxiv-submission.tar.gz .
	@rm -rf arxiv
	@echo "==> arxiv-submission.tar.gz  (upload this)"
	@echo "    contains: $(MAIN).tex, kurbanlab.sty, affiliations.tex, $(MAIN).bbl, figures/, logo/, analysis/"
	@echo "    NOT included: *.aux, *.log. references.bib IS included: arXiv ignores it,"
	@echo "    but anyone opening this tarball in Overleaf gets a working BibTeX setup."

blind:
	@sed -E 's/\\usepackage\[([^]]*)\]\{kurbanlab\}/\\usepackage[\1, blind]{kurbanlab}/' \
	     $(MAIN).tex > $(MAIN)-blind.tex
	$(LATEX) $(MAIN)-blind
	-bibtex $(MAIN)-blind
	$(LATEX) $(MAIN)-blind
	$(LATEX) $(MAIN)-blind
	@echo "==> $(MAIN)-blind.pdf  (check it: your name should appear nowhere)"

logo:
	@cd logo && sh build-logo.sh

figures:
	@cd figures && python3 make-figure.py

clean:
	@rm -f *.aux *.log *.out *.bbl *.blg *.toc *.lof *.lot *.fls *.fdb_latexmk \
	       *.synctex.gz *.nav *.snm *.vrb $(MAIN)-blind.tex
	@echo "==> cleaned"

purge: clean
	@rm -f $(MAIN).pdf $(MAIN)-blind.pdf arxiv-submission.tar.gz
	@rm -rf arxiv

